Interactive Dynamic Walking: Learning Gait Switching Policies with Generalization Guarantees

In this paper, we consider the problem of adapting a dynamically walking bipedal robot to follow a leading co-worker while engaging in tasks that require physical interaction. Our approach relies on switching among a family of Dynamic Movement Primitives (DMPs) as governed by a supervisor. We train the supervisor to orchestrate the switching among the DMPs in order to adapt to the leader's intentions, which are only implicitly available in the form of interaction forces. The primary contribution of our approach is its ability to furnish certificates of generalization to novel leader intentions for the trained supervisor. This is achieved by leveraging the Probably Approximately Correct (PAC)-Bayes bounds from generalization theory. We demonstrate the efficacy of our approach by training a neural-network supervisor to adapt the gait of a dynamically walking biped to a leading collaborator whose intended trajectory is not known explicitly.

==> extra.tex <==
% table
\begin{table}[h!]
\renewcommand{\arraystretch}{1.3}
\centering
\begin{tabular}{|c||c||c||c|}
\hline
\mbox{\boldmath$s~\textbf{(deg)}$}  & \mbox{\boldmath$ X_\mathrm{cm}(m)$} &  \mbox{\boldmath$Y_\mathrm{cm}(m)$} & \mbox{\boldmath$ s_\mathrm{cm}\textbf{(deg)}$} \\
% (N)&$(C_\mathrm{QPAC})$&(estimate)\\
\hline\hline
% 100 & 28.74\% & 5.00\%\\
% \hline
0 & 0.6789 & 0  & 0 \\
\hline
5 & 0.6770 & 0.0336 & 2.84\\
\hline
10 & 0.6730 & 0.0669 & 5.67\\
\hline
15 & 0.6670 & 0.0996 & 8.49\\
\hline
20 & 0.6590 & 0.1316 & 11.29\\
\hline
25 & 0.6492 & 0.1627 & 14.07\\
\hline
30 & 0.6377 & 0.1928 & 16.82\\
\hline
35 & 0.6246 & 0.2218 & 19.55\\
\hline
40 & 0.6100 & 0.2494 & 22.24\\
\hline
45 & 0.5940 & 0.2757 & 24.90\\
\hline
-5 & 0.6787 & -0.0339 &-2.85\\
\hline
-10 & 0.6764 & -0.0677 &-5.71\\
\hline
-15 & 0.6720 & -0.1013 &-8.57\\
\hline
-20 & 0.6655 & -0.1345 &-11.42\\
\hline
-25 & 0.6570 & -0.1671 &-14.27\\
\hline
-30 & 0.6465 & -0.1991 &-17.12\\
\hline
-35 & 0.6341 & -0.2301 &-19.95\\
\hline
-40 & 0.6199 & -0.2600 &-22.76\\
\hline
-45 & 0.6039 & -0.2887 &-25.55\\
\hline
\end{tabular}
\caption{\small The library of gait primitives. Each gait primitive $\mathcal{G}_r$ corresponds to a heading change of $s \rm(deg)$ in the robot's yaw DoF $q_1$. $(X_\mathrm{cm}(m), Y_\mathrm{cm}(m))$ denote the change in position of CoM and $(s_\mathrm{cm})$ denotes the change in orientation of the CoM.}
% Then, in the absence of the force, when the biped executes any of these primitive, the net change in the position $(X_\mathrm{cm}(m), Y_\mathrm{cm}(m))$ and orientation $(s_\mathrm{cm})$ of CoM is also provided in Table \ref{table:DMPs}.\sush{Should the headings clarify that we mean change in $X_cm$ or change in $Y_cm$? Also, instead of a table, would a plot of the CoM be more visually appealing?}}
\label{table:DMPs}
\vspace{-0.2in}
\end{table}
% table
